Learning to Select the Best Forecasting Tasks for Clinical Outcome Prediction

We propose to meta-learn an a self-supervised patient trajectory forecast learning rule by meta-training on a meta-objective that directly optimizes the utility of the patient representation over the subsequent clinical outcome prediction. This meta-objective directly targets the usefulness of a representation generated from unlabeled clinical measurement forecast for later supervised tasks. The meta-learned can then be directly used in target risk prediction, and the limited available samples can be used for further fine-tuning the model performance. The effectiveness of our approach is tested on a real open source patient EHR dataset MIMIC-III. We are able to demonstrate that our attention-based patient state representation approach can achieve much better performance for predicting target risk with low resources comparing with both direct supervised learning and pretraining with all-observation trajectory forecast.

==> append.tex <==

\section{Model Selection}



LSTM-based solutions use a hidden state size of $20$ and learning rate of $0.00075$ and $DSSM$ uses a hidden state size of $30$ and learning rate of $0.0001$. In the experiment, each timestep take $1$ hour, and the prediction rolls out to $120$ hours for both state-based hazard rate models. 
 
 
 
\section{Dataset Statistics}


  \begin{longtabu}{p{1cm}p{6cm}XXX}\caption{List of input features used in the model.} \label{tab:features} \\ \toprule
Index&
Observation Name&
LOINC code&
MIMIC specific code&
Units\\\midrule
\endhead
\bottomrule
\endfoot
0&
Heart Rate&
&
211&
bpm\\
1&
SpO2&
&
646&
percent\\
2&
Respiratory Rate&
&
618&
bpm\\
3&
Heart Rate&
&
220045&
bpm\\
4&
Respiratory Rate&
&
220210&
breaths per min\\
5&
O2 saturation pulseoxymetry&
&
220277&
percent\\
6&
Arterial BP [Systolic]&
&
51&
mmhg\\
7&
Arterial BP [Diastolic]&
&
8368&
mmhg\\
8&
Arterial BP Mean&
&
52&
mmhg\\
9&
Urine Out Foley&
&
40055&
ml\\
10&
HR Alarm [High]&
&
8549&
bpm\\
11&
HR Alarm [Low]&
&
5815&
bpm\\
12&
SpO2 Alarm [Low]&
&
5820&
percent\\
13&
SpO2 Alarm [High]&
&
8554&
percent\\
14&
Resp Alarm [High]&
&
8553&
bpm\\
15&
Resp Alarm [Low]&
&
5819&
bpm\\
16&
SaO2&
&
834&
percent\\
17&
HR Alarm [Low]&
&
3450&
bpm\\
18&
HR Alarm [High]&
&
8518&
bpm\\
19&
Resp Rate&
&
3603&
breaths\\
20&
SaO2 Alarm [Low]&
&
3609&
cm h2o\\
21&
SaO2 Alarm [High]&
&
8532&
cm h2o\\
22&
Previous WeightF&
&
581&
kg\\
23&
NBP [Systolic]&
&
455&
mmhg\\
24&
NBP [Diastolic]&
&
8441&
mmhg\\
25&
NBP Mean&
&
456&
mmhg\\
26&
NBP Alarm [Low]&
&
5817&
mmhg\\
27&
NBP Alarm [High]&
&
8551&
mmhg\\
28&
Non Invasive Blood Pressure mean&
&
220181&
mmhg\\
29&
Non Invasive Blood Pressure systolic&
&
220179&
mmhg\\
30&
Non Invasive Blood Pressure diastolic&
&
220180&
mmhg\\
31&
Foley&
&
226559&
ml\\
32&
CVP&
&
113&
mmhg\\
33&
Arterial Blood Pressure mean&
&
220052&
mmhg\\
34&
Arterial Blood Pressure systolic&
&
220050&
mmhg\\
35&
Arterial Blood Pressure diastolic&
&
220051&
mmhg\\
36&
ABP Alarm [Low]&
&
5813&
mmhg\\
37&
ABP Alarm [High]&
&
8547&
mmhg\\
38&
GCS Total&
&
198&
missing\\
39&
Hematocrit&
4544-3&
&
percent\\
40&
Potassium&
2823-3&
&
meq per l\\
41&
Hemoglobin [Mass/volume] in Blood&
718-7&
&
g per dl\\
42&
Sodium&
2951-2&
&
meq per l\\
43&
Creatinine&
2160-0&
&
mg per dl\\
44&
Chloride&
2075-0&
&
meq per l\\
45&
Urea Nitrogen&
3094-0&
&
mg per dl\\
46&
Bicarbonate&
1963-8&
&
meq per l\\
47&
Platelet Count&
777-3&
&
k per ul\\
48&
Anion Gap&
1863-0&
&
meq per l\\
49&
Temperature F&
&
678&
deg f\\
50&
Temperature C (calc)&
&
677&
deg f\\
51&
Leukocytes [\#/volume] in Blood by Manual count&
804-5&
&
k per ul\\
52&
Glucose&
2345-7&
&
mg per dl\\
53&
Erythrocyte mean corpuscular hemoglobin concentration [Mass/volume] by Automated count&
786-4&
&
percent\\
54&
Erythrocyte mean corpuscular hemoglobin [Entitic mass] by Automated count&
785-6&
&
pg\\
55&
Erythrocytes [\#/volume] in Blood by Automated count&
789-8&
&
per nl\\
56&
Erythrocyte mean corpuscular volume [Entitic volume] by Automated count&
787-2&
&
fl\\
57&
Erythrocyte distribution width [Ratio] by Automated count&
788-0&
&
percent\\
58&
Temp/Iso/Warmer [Temperature degrees C]&
&
8537&
deg f\\
59&
FIO2&
&
3420&
percent\\
60&
Magnesium&
2601-3&
&
mg per dl\\
61&
CVP Alarm [High]&
&
8548&
mmhg\\
62&
CVP Alarm [Low]&
&
5814&
mmhg\\
63&
Calcium [Moles/volume] in Serum or Plasma&
2000-8&
&
mg per dl\\
64&
Phosphate&
2777-1&
&
mg per dl\\
65&
FiO2 Set&
&
190&
torr\\
66&
Temp Skin [C]&
&
3655&
in\\
67&
pH&
11558-4&
&
u\\
68&
Temperature Fahrenheit&
&
223761&
deg f\\
69&
Central Venous Pressure&
&
220074&
mmhg\\
70&
Inspired O2 Fraction&
&
223835&
percent\\
71&
PAP [Systolic]&
&
492&
mmhg\\
72&
PAP [Diastolic]&
&
8448&
mmhg\\
73&
Calculated Total CO2&
34728-6&
&
meq per l\\
74&
Oxygen [Partial pressure] in Blood&
11556-8&
&
mmhg\\
75&
Base Excess&
11555-0&
&
meq per l\\
76&
Carbon dioxide [Partial pressure] in Blood&
11557-6&
&
mmhg\\
77&
PTT&
3173-2&
&
s\\
78&
Deprecated INR in Platelet poor plasma by Coagulation assay&
5895-7&
&
ratio\\
79&
PT&
5902-2&
&
s\\
80&
Temp Axillary [F]&
&
3652&
deg f\\
81&
Day of Life&
&
3386&
\\
82&
Total Fluids cc/kg/d&
&
3664&
\\
83&
Present Weight (kg)&
&
3580&
kg\\
84&
Present Weight (lb)&
&
3581&
cm h2o\\
85&
Present Weight (oz)&
&
3582&
cm h2o\\
86&
Fingerstick Glucose&
&
807&
mg per dl\\
87&
PEEP set&
&
220339&
cm h2o\\
88&
Previous Weight (kg)&
&
3583&
kg\\
89&
Weight Change (gms)&
&
3692&
g\\
90&
PEEP Set&
&
506&
cm h2o\\
91&
Mean Airway Pressure&
&
224697&
cm h2o\\
92&
Tidal Volume (observed)&
&
224685&
ml\\
93&
Resp Rate (Total)&
&
615&
bpm\\
94&
Minute Volume Alarm - High&
&
220293&
l per min\\
95&
Minute Volume Alarm - Low&
&
220292&
l per min\\
96&
Apnea Interval&
&
223876&
s\\
97&
Minute Volume&
&
224687&
l per min\\
98&
Paw High&
&
223873&
cm h2o\\
99&
Peak Insp. Pressure&
&
224695&
cm h2o
\end{longtabu}

\section{Additional Experiment Results}

\begin{table}[h!]
\centering
\begin{center}
\begin{tabular}{c  p{1.8cm}   p{1.8cm} p{1.8cm}   p{1.8cm}   p{1.8cm}}  \\
\toprule 
                & C-Index& AUC-ROC@24 & AP@24 & AUC-ROC@48 &  AP@48 \\
 \hline
Deep Cox     &  0.771 [0.750, 0.814] &0.835 [0.782, 0.901] & 0.094 [0.047, 0.185] & 0.828 [0.793, 0.858] & 0.106 [0.065, 0.183]  \\ 
 \hline                 
LSTM + Exp  & 0.790      [0.746, 0.819] & 0.851 [0.777, 0.909] & 0.260 [0.126, 0.425] & 0.835 [0.760, 0.905] & 0.262 [0.154, 0.372]\\ 
 \hline                 
LSTM + State    & 0.799  [0.769, 0.841]& 0.890 [0.835, 0.934] & 0.313 [0.220, 0.470] & 0.867 [0.800, 0.927] & 0.362 [0.260, 0.498] \\ 
 \hline 
DSSM + Exp     & 0.797 [0.758, 0.820] & 0.883 [0.836, 0.930] & 0.298 [0.165, 0.474] & 0.875 [0.830, 0.922] &   0.309 [0.164, 0.450]\\ 
 \hline 
DSSM + State    & \textbf{0.809} [0.775, 0.831] & \textbf{0.896} [0.834, 0.955] & \textbf{0.357} [0.169, 0.553] & \textbf{0.881} [0.837, 0.908] & \textbf{0.365} [0.280, 0.452] \\ 
 \bottomrule
\end{tabular}
\end{center}
\caption{Time-to-Mortality Prediction Results.}
\label{table:survival_result}
\end{table}

    
\begin{table}[h!]
\centering
\vspace{-5mm}
\scriptsize
\begin{tabular}{lp{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}}  \\
\toprule 
& 1\ && 10\%&&100\&& 
 \midrule                
  &  AUC & AP & AUC & AP& AUC & AP& 
\cmidrule{1-7}
Supervised (SUP) & 0.7382(0.0165)& 0.0477(0.0043)& 0.8529(0.0164) & 0.1271(0.0117) & 0.8999(0.0079) & 0.2677(0.0286) 
\\ 
Pretrain w/All  (with Freeze E )&	0.6264(0.0290) & 0.0389(0.0091)&	0.7699(0.0088) & 0.0657(0.0047) & 0.8161(0.0201) & 0.1101(0.0138) \\ 
Pretrain w/All  (with Finetune )&	0.8091(0.0102) & 0.0736(0.0073)& 0.8531(0.0129) & 0.1542(0.0156) & 0.8995(0.0107) & 0.2683(0.0194) \\ 

Pretrain w/Cotrain  (with Freeze E )&	0.7522(0.018) & 0.0578(0.0066)&	0.8560(0.0103) & 0.1484(0.0237) & 0.8982(0.0106) & 0.2608(0.0270) \\ 
Pretrain w/Cotrain  (with Finetune )&	0.7253(0.0141) & 0.0567(0.0074)& 0.8542(0.0142) & 0.1352(0.0097) & 0.9027(0.0090) &  0.2621(0.0286) \\ 

PATS [1000/5] (with Freeze E )&	0.7867(0.0104) & 0.0822(0.0051) &	0.8326(0.0098) & 0.1083(0.0103) & 0.8634(0.0097) & 0.1354(0.0143) \\ 
PATS [1000/5] (with Finetune )&	0.8302(0.0153) & 0.0945(0.0043) & \textbf{0.8822}(0.0125) & 0.1655(0.0173) & 0.9047(0.0116) &  0.2634(0.0273) \\ 
PATS [500/10] (with Freeze E )&	0.7550(0.0036) & 0.0528(0.0055) & 0.8305(0.0071) & 0.1071(0.0071) & 0.8664(0.0111) & 0.1421(0.011) \\ 
PATS [500/10] (with Finetune )&	0.8246(0.0159) & 0.0977(0.0092)& 0.8737(0.0130) & 0.1590(0.0263) & 0.9069(0.0139) &  0.2613(0.0179) \\ 
PATS [100/50] (with Freeze E )&	0.7695(0.0144) & 0.0665(0.0093) & 0.8372(0.0116) & 0.1264(0.0137) & \textbf{0.9088}(0.0078) & 0.2567(0.0216)\\ 
PATS [100/50] (with Finetune )&	0.8311(0.0159) & \textbf{0.0979}(0.0131) & 0.8708(0.0124) & 0.1571(0.0200) & 0.9055(0.0090) & 0.2739(0.0278)  \\ 
PATS [50/100] (with Freeze E )&	 0.797(0.0168) & 0.0708(0.0041) & 0.8333(0.0094) &  0.1039(0.0100) & 0.8492(0.0115)  &  0.1549(0.0185) \\ 
PATS [50/100] (with Finetune )&	\textbf{0.8332}(0.0176) & 0.0947(0.0071) & 0.8633(0.0124) & \textbf{0.1683}(0.0245) & 0.9030(0.0110) & 0.2691(0.0341) \\ 
PATS [10/500] (with Freeze E )&	  0.7312(0.0158) & 0.0609(0.0081) & 0.8314(0.0114) &  0.1094(0.0117) & 0.8422(0.0063)  &  0.1371(0.0164)\\ 
PATS [10/500] (with Finetune )&	0.8238(0.0141) &  0.0880(0.0057) & 0.8733(0.0096) & 0.1504(0.0183) & 0.9045(0.0117) & \textbf{0.2909}(0.0339) \\ 
Pretrain w/top 20 Tasks (with finetune) 
&0.8097(0.0132)
& 0.08299(0.0106)&0.8497(0.01095)&0.1071(0.02565)& 0.9041(0.01149)& 0.2735(0.02487) \\
Pretrain w/o top 20 Tasks (with finetune) &0.7717(0.0192)&0.074(0.006982)&0.8231(0.01419)& 0.1006(0.01296)	&0.8921(0.01199)& 0.2316(0.02805)	\\ 
\bottomrule
\end{tabular}
\caption{\small Mortality Prediction. Parentheses denote standard error.}
\label{tab:forecast}
\end{table}

\begin{table}[h!]
\centering
\vspace{-5mm}
\scriptsize
\begin{tabular}{lp{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}}  \\
\toprule 
& 1\ && 10\%&&100\&& 
 \midrule                
  &  AUC & AP & AUC & AP& AUC & AP& 
\cmidrule{1-7}
Supervised (SUP) & 0.7304(0.0224)& 0.03537(0.0058)& 0.7545(0.0401) & 0.0865(0.0259) &  0.886(0.0264) & 0.2004(0.0526)
\\ 
Pretrain w/All  (with Freeze E )& 0.6487(0.0224) & 0.0544(0.0180)&	0.6210(0.0376) & 0.0397(0.0121) & 0.6051(0.0214) & 0.0341(0.0123) \\ 
Pretrain w/All  (with Finetune )& 0.7778(0.03098)& 0.09533(0.03406)	& 0.7721(0.0286)& 0.06388(0.02163) & 0.8814(0.03022)& 0.2161(0.05254) \\
Pretrain w/Cotrain  (with Freeze E ) & 0.7062(0.03076)& 0.05085(0.01779)	& 0.773(0.02941)&  0.09392(0.02018)	& 0.8866(0.02621)	& 0.2231(0.05482) \\
Pretrain w/Cotrain  (with Finetune)
& 0.7184(0.0413)&0.05489(0.01977)	& 0.7235(0.03127)& 0.08238(0.02162)	&0.8921(0.01899)& 0.2235(0.05756) \\ 
PATS [1000/5] (with Freeze E )& 0.7546(0.02991)&0.06569(0.01595)&0.769(0.02397)&0.08365(0.03106)	&0.7819(0.02246)& 0.06636(0.01911) \\ 
PATS [1000/5] (with Finetune )& 0.8364(0.02016) & 0.08009(0.0193)	&0.8331(0.01809)&0.1092(0.03153)& 0.8891(0.02399)& 0.185(0.03566) \\
PATS [500/10] (with Freeze E ) &0.8056(0.01878)& 0.07709(0.02873)	& 0.7698(0.02036)& 0.08709(0.03427)	& 0.8113(0.0196)& 0.1032(0.03372) \\
PATS [500/10] (with Finetune )& 0.8241(0.01724)& 0.07205(0.01163)& 0.8198(0.02952) &0.09834(0.03043) & 0.8984(0.01585)	& 0.1957(0.05164) \\
PATS [100/50] (with Freeze E )&	 0.7754(0.01956) & 0.05049(0.007348)& 0.7765(0.01411)& 0.09022(0.02611) & 0.7857(0.02679)	& 0.07073(0.018) \\
PATS [100/50] (with Finetune )&	 0.8383(0.02228)& 0.05888(0.01277)& 0.83(0.03127)& 0.09477(0.02344)	& 0.8909(0.02465)& 0.1928(0.03527) \\
Pretrain w only BP (with finetune) & 0.812(0.01413)	&0.06106(0.009006)	&0.8239(0.02115)& 0.09691(0.021)& 0.8989(0.02114)& 0.2497(0.06224) \\
Pretrain w/o BP (with finetune) &  0.7877(0.01956) & 0.0934(0.02666)& 0.7807(0.02711) & 0.1007(0.02958) &  0.8903(0.02471)& 0.1101(0.03602)\\ 
PATS with mortality then transfer &  0.8416(0.01854) & 0.08335(0.01791) & 0.8473(0.01984)&  0.1239(0.03495) &&&\\ 
 \bottomrule
\end{tabular}
\caption{\small Shock Prediction. Parentheses denote standard error.}
\label{tab:forecast}
\end{table}

\begin{table}[h!]
\centering
\vspace{-5mm}
\scriptsize
\begin{tabular}{lp{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}}  \\
\toprule 
& 1\ && 10\%&&100\&& 
 \midrule                
  &  AUC & AP & AUC & AP& AUC & AP& 
\cmidrule{1-7}

Supervised (SUP) &0.7447(0.01507)& 0.04724(0.00278)	& 0.8495(0.01522)	 & 0.126(0.01412)& 0.9015(0.01121)& 0.2042(0.01725) \\
Pretrain w/All  (with Freeze E )& 0.6001(0.01336) & 0.05807(0.01839) & 0.6622(0.01356) & 0.04993(0.009756)	& 0.7673(0.008322) & 0.08569(0.008383)\\
Pretrain w/All  (with Finetune )&0.771(0.02134)& 0.07445(0.01341)& 0.8282(0.01223)& 0.113(0.01382)	& 0.907(0.006776)& 0.2233(0.01255) \\
Pretrain w/Cotrain  (with Freeze E ) &  0.6997(0.02696)& 0.0506(0.007365) & 0.8455(0.01476)& 0.1089(0.01232)	& 0.8966(0.007231) & 0.2163(0.0198) \\
Pretrain w/Cotrain  (with Finetune)&  0.7478(0.02161)& 0.07591(0.01108)& 0.8493(0.01273)& 0.1154(0.01486)	& 0.899(0.009563)	& 0.2266(0.01669) \\
PATS [1000/5] (with Freeze E )& 0.7677(0.02257)& 0.07225(0.002604)		& 0.8287(0.01664) & 0.1459(0.02802)	& 0.8539(0.011)& 0.1509(0.02957) \\
PATS [1000/5] (with Finetune )&  0.8184(0.01677)& 0.1051(0.009701)& 0.8626(0.01826)&  0.1371(0.004191)& 0.908(0.009835)	& 0.2278(0.02516) \\
PATS [500/10] (with Freeze E ) &0.7895(0.01654)& 0.07266(0.008939)& 0.8268(0.01729)	& 0.1062(0.006456)	& 0.8569(0.01266)	& 0.1268(0.01604) \\
PATS [500/10] (with Finetune )& 0.8223(0.01722)	& 0.07933(0.007105) & 0.8607(0.0149) & 0.1445(0.01434)& 0.9066(0.005939)& 0.2143(0.02077) \\
PATS [100/50] (with Freeze E )&	 0.7865(0.02063) & 0.07016(0.01161) & 0.8236(0.01882) & 0.1215(0.008221)	& 0.8617(0.008898)&  0.1517(0.02946) \\
PATS [100/50] (with Finetune )&	 0.8231(0.01806)& 0.08497(0.00619)& 0.8579(0.02164)& 0.139(0.01525)	&		 0.91(0.01133) &	0.2497(0.01782) \\
Pretrain w only CR (with finetune) & 0.7359(0.009682)& 0.04501(0.00861) & 0.8334(0.01721)& 0.09866(0.02495)	& 0.8973(0.01206)& 0.2093(0.03494) \\
Pretrain w/o CR (with finetune) &   0.8022(0.01686) & 0.06676(0.01559) & 0.8506(0.0178) & 0.1368(0.0192)	& 0.8964(0.01221)	& 0.2489(0.02257) \\
PATS with mortality then transfer & 0.8333(0.01695)& 0.1044(0.01227)	& 0.8685(0.01911)& 0.1515(0.007944)&&&\\ 
 \bottomrule
\end{tabular}
\caption{\small Kidney Failure. Parentheses denote standard error.}
\label{tab:forecast}
\end{table}


==> tikz.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

